CORE: A Few-Shot Company Relation Classification Dataset for Robust Domain Adaptation

We introduce CORE, a dataset for few-shot relation classification (RC) focused on company relations and business entities. CORE includes 4,708 instances of 12 relation types with corresponding textual evidence extracted from company Wikipedia pages. Company names and business entities pose a challenge for few-shot RC models due to the rich and diverse information associated with them. For example, a company name may represent the legal entity, products, people, or business divisions depending on the context. Therefore, deriving the relation type between entities is highly dependent on textual context. To evaluate the performance of state-of-the-art RC models on the CORE dataset, we conduct experiments in the few-shot domain adaptation setting. Our results reveal substantial performance gaps, confirming that models trained on different domains struggle to adapt to CORE. Interestingly, we find that models trained on CORE showcase improved out-of-domain performance, which highlights the importance of high-quality data for robust domain adaptation. Specifically, the information richness embedded in business entities allows models to focus on contextual nuances, reducing their reliance on superficial clues such as relation-specific verbs. In addition to the dataset, we provide relevant code snippets to facilitate reproducibility and encourage further research in the field.

==> Tables/results_semeval.tex <==
\begin{table}
\centering
\scalebox{0.8}{
    \begin{tabular}{llll}
    \hline
    \textbf{Domain} & \textbf{Model} & \textbf{5-1} & \textbf{5-5} \\
    \hline
    In-domain & Proto-BERT & &  \\
    & BERT-Pair &  &  \\
    & BERT\textsubscript{EM} &  & \\
    & BERT-Prompt &  &  \\
    & HCRP &  &  \\
    \hline
    CORE & Proto-BERT &  &  \\
    & BERT-Pair &  &  \\
    & BERT\textsubscript{EM} & 23.28 / 30.83 & 30.72 / 42.71 \\
    & BERT-Prompt & \underline{34.41} / \textbf{39.06} & \underline{46.61} / 35.15 \\
    & HCRP & 16.57 / 36.36 & 21.89 / \textbf{48.48} \\
    \hline
    FewRel & Proto-BERT &  &  \\
    & BERT-Pair &  &  \\
    & BERT\textsubscript{EM} & 23.45 / 29.48 & 29.52 / 37.11 \\
    & BERT-Prompt & \underline{25.63} / \underline{39.54} & \underline{31.49} / 38.04 \\
    & HCRP & 15.51 / 34.27 & 19.86 / \underline{44.18} \\
    \hline
    TACRED & Proto-BERT &  &  \\
    & BERT-Pair &  &  \\
    & BERT\textsubscript{EM} & 19.36 / 23.72 & 21.37 / 25.52 \\
    & BERT-Prompt & \underline{36.04} / \underline{38.03} & \textbf{47.49} / \underline{33.18} \\
    & HCRP & 17.82 / 31.93 & 47.19 / 30.35 \\
    \hline
    \end{tabular}}
    \caption{Micro F1 / Macro F1 for in-domain and out-of-domain models evaluated on SemEval.}
    \label{tab:results_semeval}
\end{table}
